Simplicial Embeddings in Self-Supervised Learning and Downstream Classification

Simplicial Embeddings (SEM) are representations learned through self-supervised learning (SSL), wherein a representation is projected into $L$ simplices of $V$ dimensions each using a softmax operation. This procedure conditions the representation onto a constrained space during pretraining and imparts an inductive bias for group sparsity. For downstream classification, we formally prove that the SEM representation leads to better generalization than an unnormalized representation. Furthermore, we empirically demonstrate that SSL methods trained with SEMs have improved generalization on natural image datasets such as CIFAR-100 and ImageNet. Finally, when used in a downstream classification task, we show that SEM features exhibit emergent semantic coherence where small groups of learned features are distinctly predictive of semantically-relevant classes.

==> 3.2-Theory_1.tex <==

\subsection{SEM improvement on the generalization of the downstream classifier}
% \subsection{Theoretical bound on the downstream classifier}
\label{sec-theory}

In this subsection, we  mathematically analyze the effect of using SEM for downstream classification. We theoretically demonstrate the benefit of training a downstream classifier with SEM normalized input compared to a baseline classifier with unnormalized input. %We focus on classification as the downstream task and show that
In summary, we show that: (1)  there is a trade-off between the training loss and the generalization gap, which is controlled by the value of $\tau_d$, (2) SEM can improve the base model performance when we attain good balance in this trade-off, and (3) the improvement due to SEM is expected to increase or stay constant as $L$ and $V$ increase. In the remaining of this subsection, we consider $\tau = \tau_d$.

\textbf{Notation} %To formally prove and state this, we first introduce the notation.
We consider a training dataset $S=(z^{(i)},y^{(i)})_{i=1}^n$ of $n$ samples that is used for supervised training of a classifier using the representation $z$, which are extracted from the pre-trained model\footnote{In this subsection, we assume that the extracted representation is $z$, the embedder's output}, and the corresponding label $y\in\Ycal$ with $\Ycal$ the set of possible labels. We assume that $z\in \Zcal = [-1,+1]^{L\times V}$, that is we assume that $z$ is bounded to $[-1,+1]$ and that $z$ is partitioned into $L$ vectors $z_i$, each of $V$ dimensions.
Let $g$ represent the downstream classifier trained on the representation. We can define a baseline model where $g$ is trained without normalization as $f_{\base}(z) = g(z)$ and the corresponding model trained with the SEM normalization of the representation's features as $f_{\SD{\tau}}(z)=(g\circ\sigma_{\tau})(z)$.
%To understand the quality of the final model after supervised training of the classifier, 
To compare the quality of the  base model and the model with SEM normalization, we analyze the generalization gap $
\EE_{z,y}[l(f(z) ,y)]   - \frac{1}{n} \sum_{i=1}^n l(f(z^{(i)}),y^{(i)}) $ for each $f \in \{f_{\SD(\tau)}^S, f_\base^S\}$,
where $l:\RR \times\Ycal\rightarrow \RR_{\ge 0}$ is the per-sample loss and $f^S_{\SD(\tau)}$, $f^S_\base$ are the models obtained from fitting the dataset $S$. 

%To simplify the notation, we consider the normalization to $[-1,+1]$; i.e., the encoder's output $z \in \Zcal = [-1,+1]^{L\times V}$.
Next, we define $q\in [-1,+1]^V$, which can be understood as a partition $z_i$. We can define
$\Qcal_{i}= \{q :  i=\argmax _{j \in [V]} q_{j}\}$ that represents $V$ partitions of the space $[-1,+1]^V$. In words, the partition $\Qcal_{i}$ is the set where the elements $q_i>q_j, \forall j\neq i$. We use the partitions $\Qcal_i$ to define the following measure that allows us to understand the effect of SEM normalization on the vectors $z_i$ which are given to the classifier $g$ and thus to compare $f^S_\SD$ and $f^S_\base$, a model with and without SEM normalization respectively:
\begin{equation}
\varphi(\sigma_f) = \sup_{i\in [V]}\sup_{q,q' \in Q_i}\|\sigma_{f}(q)-\sigma_{f}(q')\|_2
\end{equation}
where $\sigma_f\in\{\sigma_{f^S_\text{SEM}(\tau)}, \sigma_{f^S_\base}\}$ are the function applied on the representations (i.e. $z_i$) for $f^S_\SD$ and $f^S_\base$ respectively and then given to $g$. They are defined as follows:  $\sigma_{f_{\SD(\tau)}^{S}}=\sigma_{\tau}$ and $\sigma_{f_\base^{S}}$ is the identity function.
% $
% \varphi(f_\base^{S})=\sup_{i\in [V]}\sup_{q,q' \in Q_i}\sum_{t=1}^n\|q-q'\|_2^2, $
% and
% $
% \varphi(f_{\SD(\tau)}^{S})= \sup_{i\in [V]}\sup_{q,q' \in Q_i}\sum_{t=1}^n\|\sigma_{\tau}(q)-\sigma_{\tau}(q')\|_2^2
% $,
Here, $\sigma_{\tau}(q)_{j}= \frac{e^{q_{j}/\tau}}{\sum_{t=1}^V e^{q_{t}/\tau}}$ for $j=1,\dots,V$. Intuitively, $\varphi$ is an upper bound on the expressivity of a vector $z_i$ and depends on $V$ and also $\tau$ for the SEM normalized representations. % TODO: Give an intuitive view of $\varphi$.

We also make the following assumptions. %for our theorem to hold true.
% Can we put the following assumptions on the Appendix?
We assume that there exists $\Delta>0$ such that for any $i \in [L]$, if $k=\argmax_{j\in[V]} z_{ij}$, then $z_{ik} \ge z_{ij}+\Delta$ for any $j \neq k$.
Since $\Delta$ can be arbitrarily small (e.g., much smaller than machine precision),
this assumption typically holds in practice.
Next, we define  $B$ to be the upper bound on the per-sample loss such that  $l(f(z),y)\le B$ for all $f \in \Hcal$ and for all $(z ,y)\in \Zcal \times \Ycal$, where  $\Hcal$ is the union of the hypothesis spaces of $f_{\SD(\tau)}$ and $f_{\base}$. For example, $B=1$ for the 0-1 loss. 


% TODO: Verify with Kenji that this modification is correct
Finally, we define $\Gcal_S$ to be the set of classifiers $g$ returned by the training algorithm using dataset $S$, and $R$ to be the Lipschitz constant of $l_y \circ g$ for all $y \in\Ycal$ and $g \in \Gcal_{S}$; i.e., $|(l_{y}\circ g)^{}(\sigma_f(z))-(l_{y}\circ g)(\sigma_f(z'))|\le R\|\sigma_f(z)-\sigma_f(z')\|_F$, where 
$l_y(g\circ\sigma_f(z))=l(g\circ\sigma_f(z),y)$. We denote by $c>0$ a constant in  $(n, f, \Hcal, \delta, \tau, S)$. %$(n,f,\Hcal,\delta, \Hcal,\tau,S)$. 

% Finally, we define $\Gcal_S$ to be the set of classifiers $g$ returned by the training algorithm using dataset $S$, and $R$ to be the Lipschitz constant of $l_y \circ g$ for all $y \in\Ycal$ and $g \in \Gcal_{S}$; i.e., $|(l_{y}\circ g)^{}(z)-(l_{y}\circ g)(z')|\le R\|z-z'\|_F$, where  $l_y(q)=l(q,y)$. We denote by $c>0$ a constant in  $(n,f,\Hcal,\delta, \Hcal,\tau,S)$. 

Using the established notation, Theorem~\ref{thm:1} illuminates the advantage of SEM and the effect of the hyper-parameter $\tau$ on the performance of the downstream classifier. We present the proof in Appendix~\ref{sec-proof} and we present empirical evidence of the theorem's prediction in Figure~\ref{fig:fsem_compare}.
\begin{restatable}{theorem}{thma} \label{thm:1}
 Let $V\ge 2$. For any $\delta>0$,  with  probability at least $1-\delta$, the following holds for any $f_{S}\in \{f_{\SD(\tau)}^S, f_\base^S\}$: \vspace{-10pt}
\begin{align} \label{eq:4}
\EE_{z,y}[l(f_{S}(z) ,y)]   \le\frac{1}{n} \sum_{i=1}^n l(f_{S}(z^{(i)}),y^{(i)}) 
 \nonumber  + R\sqrt{L \varphi(\sigma_{f_{S}})}+ c \sqrt{\frac{\ln(2/\delta)}{n}}. \vspace{-10pt}
\end{align}
Moreover, 
\begin{align*}
\varphi(\sigma_{f_{\SD(\tau)}^{S}}) \rightarrow 0 \ \ \text{ as } \tau \rightarrow 0 \quad \text{and}\quad \varphi(\sigma_{f_{\SD(\tau)}^{S}})-\varphi(\sigma_{f_{\base}^{S}})\le  \frac{3}{4}(1-V)<0 \ \ \ \forall \tau >0. 
\end{align*}
\end{restatable}
The first statement of \Cref{thm:1} shows that the expected loss is bounded by the three terms: the training loss $\frac{1}{n} \sum_{i=1}^n l(f_{S}(z^{(i)}),y^{(i)}) $, the second term $R\sqrt{L \varphi(f_{S})}$, and the third term $c \sqrt{\frac{\ln(2/\delta)}{n}}$. Since $c$ is a constant in $(n, f, \Hcal, \delta, \tau, S)$, % $(n,f,\Hcal,\delta, \Hcal,\tau,S)$,
the third term goes to zero as $n\rightarrow \infty$ and is the same with and without SEM. Thus, for the purpose of assessing the impact of SEM,  we can focus on the second term, where a difference arises. 

\Cref{thm:1} shows that  $R\sqrt{L \varphi(f_{S})}$ goes to zero with SEM; i.e.,  $\varphi(f_{\SD(\tau)}^{S}) \rightarrow 0 \text{ as } \tau \rightarrow 0$. Also, for any $\tau>0$, the second term with SEM is strictly smaller than that without SEM as $\varphi(f_{\SD(\tau)}^{S})-\varphi(f_{\base}^{S})\le  \frac{3}{4}(1-V)<0$ and demonstrates that the improvement due to SEM is expected to asymptotically increase as $V$ increases. Also, $L$ is a multiplicative constant of $\varphi$ which shows that as $L$ increases, the expect improvement due to SEM is also expected to be higher.

Overall, \Cref{thm:1} shows the benefit of SEM as well as the trade-off with $\tau$. When $\tau \rightarrow 0$, the second term goes to zero, but the training loss (the first term) can increase due to the reduction in expressivity and increased difficulty in optimization. Thus, $\tau$ should be chosen to optimally balance this trade-off.

==> 7-Limitations.tex <==
\section{Limitations and broader impact}
\label{limitation}
We observe that improved model performance is tied to large representation size. With a sufficiently large representation, using small $\tau_d$ effectively discretizes the features and yielded the best accuracy on CIFAR-100. For ImageNet, our optimal temperature $\tau_d$ was still quite high, indicating that the optimal representation size is likely larger than what could fit on our hardware. This demonstrates that very large embeddings might be necessary to achieve the full potential of SEM, especially for large datasets with complex semantics like ImageNet. This may limit its use, especially when working under hardware constraints.
%This work studies the effect on projecting the data into simplicial embeddings for pre-training and downstream tasks and thus apply generally to positive and negative applications. 
